Multifactorial Evolutionary Algorithm For Clustered Minimum Routing Cost Problem

Minimum Routing Cost Clustered Tree Problem (CluMRCT) is applied in various fields in both theory and application. Because the CluMRCT is NP-Hard, the approximate approaches are suitable to find the solution for this problem. Recently, Multifactorial Evolutionary Algorithm (MFEA) has emerged as one of the most efficient approximation algorithms to deal with many different kinds of problems. Therefore, this paper studies to apply MFEA for solving CluMRCT problems. In the proposed MFEA, we focus on crossover and mutation operators which create a valid solution of CluMRCT problem in two levels: first level constructs spanning trees for graphs in clusters while the second level builds a spanning tree for connecting among clusters. To reduce the consuming resources, we will also introduce a new method of calculating the cost of CluMRCT solution. The proposed algorithm is experimented on numerous types of datasets. The experimental results demonstrate the effectiveness of the proposed algorithm, partially on large instances

==> glosaries.tex <==
\newacronym{ga}{GA}{Genetic Algorithm}
\newacronym{ea}{EA}{Evolutionary Algorithm}
\newacronym{gp}{GP}{Genetic Programming}
\newacronym{ant}{ACO}{Ant Colony Optimization}
\newacronym{grasp}{GRASP}{Greedy Randomized Adaptive Search Procedure}
\newacronym{de}{DE}{Differential Evolution Algorithm}
\newacronym{pso}{PSO}{Particles Warm Optimization Algorithm}
\newacronym{rmp}{rmp}{Probability of Random Mating}
\newacronym{ltga}{LTGA}{Linkage Tree Genetic Algorithm}
\newacronym{rga}{RGA}{Randomized Greedy Algorithm}

\newacronym{sto}{STO}{single-tasking of Genetic Algorithm}
\newacronym{uss}{USS}{Unified Search Space}
\newacronym{mfo}{MFO}{Multifactorial Optimization}
\newacronym{mfea}{MFEA}{Multifactorial Evolutionary Algorithm}

\newacronym{cluspt}{CluSPT}{Clustered Shortest-Path Tree Problem}
\newacronym{clumrct}{CluMRCT}{Minimum Routing Cost Clustered Tree Problem}
\newacronym{clutsp}{CluTSP}{Clustered Traveling Salesman Problem}
\newacronym{clusteiner}{CluSteiner}{Clustered Steiner Tree Problem}
\newacronym{interclumrct}{InterCluMRCT}{Minimum Inter-cluster Routing Cost Clustered Tree Problem}

\newacronym{ftsp}{FTSP}{Family Traveling Salesman Problem}
\newacronym{gtsp}{GTSP}{Generalized Traveling Salesman Problem}
\newacronym{tsp}{TSP}{Traveling Salesman Problem}
\newacronym{steinertp}{STP}{Steiner Tree Problem}
\newacronym{vrp}{VRP}{Vehicle Routing Problem}
\newacronym{cvrp}{CVRP}{Capacitated Vehicle Routing Problem}

\newacronym{rpd}{RPD}{Relative Percentage Differences}

==> sections/other/preamble.tex <==
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\setcopyright{acmcopyright}
\copyrightyear{2019}
\acmYear{2019}
\acmDOI{10.1145/1122445.1122456}

\acmConference[SoICT 2019]{SoICT 2019: Symposium on Information and Communication Technology}{June 03--05, 2018}{Hanoi - Halong Bay, VN}
\acmBooktitle{SoICT 2019: Symposium on Information and Communication Technology,
  Dec 4-6, 2019, Hanoi - Halong Bay, VN}
\acmPrice{15.00}
\acmISBN{978-1-4503-9999-9/18/06}

\acmSubmissionID{123-A56-BU3}



==> sections/result/table.tex <==
\newpage
\onecolumn
\begin{landscape}
  \begin{multicols}{2}
  \medskip\setbox\ltmcbox\vbox{\makeatletter\col@number\@ne
    \input{Results/Type1}\unskip\unpenalty\unpenalty
  }\unvbox\ltmcbox

  \medskip\setbox\ltmcbox\vbox{\makeatletter\col@number\@ne
    \input{Results/Type34}\unskip\unpenalty\unpenalty
  }\unvbox\ltmcbox

  \medskip\setbox\ltmcbox\vbox{\makeatletter\col@number\@ne
    \input{Results/Type5}\unskip\unpenalty\unpenalty
  }\unvbox\ltmcbox

  \medskip\setbox\ltmcbox\vbox{\makeatletter\col@number\@ne
    \input{Results/Type6}\unskip\unpenalty\unpenalty
  }\unvbox\ltmcbox
  \end{multicols}
\end{landscape}

